Distributed Asynchronous Mixed-Integer Linear Programming with Feasibility Guarantees

In this paper we solve mixed-integer linear programs (MILPs) via distributed asynchronous saddle point computation. This work is motivated by the MILPs being able to model problems in multi-agent autonomy, such as task assignment problems and trajectory planning with collision avoidance constraints in multi-robot systems. To solve a MILP, we relax it with a linear program approximation. We first show that if the linear program relaxation satisfies Slater's condition, then relaxing the problem, solving it, and rounding the relaxed solution produces a point that is guaranteed to satisfy the constraints of the original MILP. Next, we form a Lagrangian saddle point problem that is equivalent to the linear program relaxation, and then we regularize the Lagrangian in both the primal and dual spaces. Doing so gives a regularized Lagrangian that is strongly convex-strongly concave. We then develop a parallelized algorithm to compute saddle points of the regularized Lagrangian, and we show that it is tolerant to asynchrony in the computations and communications of primal and dual variables. Suboptimality bounds and convergence rates are presented for convergence to a saddle point. The suboptimality bound accounts for (i) the error induced by regularizing the Lagrangian and (ii) the suboptimality gap between the solution to the original MILP and the solution to its relaxed form. Simulation results illustrate these theoretical developments in practice, and show that relaxation and regularization combined typically have only a mild impact on the suboptimality of the solution obtained.

==> equalityForm.tex <==
\begin{problem}
    \emph{(Original MILP)\label{prob:Original-MILP}}
    \end{problem}
    \begin{align*}
    \underset{(x,y)\in\mathbb{R}^{n}\times\mathbb{Z}^{m}}{\text{minimize}} & \enskip a^{T}x+d^{T}y\\
    \text{subject to} & \enskip Hx+By\leq h\\
                      & \enskip Cx+Dy = \theta\\
     & y^{\ell}\leq y\leq y^{u}, x\in X,
    \end{align*}
    \emph{where $a\in \mathbb{R}^{n}, d \in \mathbb{R}^{m}, H\in \mathbb{R}^{p\times m}, B \in \mathbb{R}^{p\times m}, h\in\mathbb{R}^{p}, C\in \mathbb{Q}^{q\times n}, 
    D \in \mathbb{Q}^{q\times m}, \theta \in \mathbb{R}^{q}$,  $\mathbb{R}$ are the real numbers, and $\mathbb{Q}$ are the rational numbers.}
    
    Use any algorithm to find the Hermite normal form of the equality matrices if $D \neq 0$.
    \begin{prop}\label{prop:propHermite}\cite{neumann2021inner}[Lemma 6.2.3]
        Let $(K,0)$ be the Hermite normal form of $D$ with $DU=(K,0)$, let $K^{-1}\theta$ be integral, and define $U_{1}:=U_{:,1:q}$, $U_{2}:=U_{:,q:m}$,
        the identity
        \begin{align*}
             \{y\in \mathbb{Z}^{m}|Dy=\theta\}=\{U_{1}K^{-1}\theta+U_{2}\eta|\eta\in \mathbb{Z}^{m-q}\},
        \end{align*}
        holds.
    \end{prop}
    When this identity holds, we have an equivalent mixed-integer program formulation to Problem \ref{prob:Original-MILP}.
    
    \noindent \textbf{Assumption 1}\emph{ There are no continuous dependent variables.}
    \begin{lem}\label{lem:reparam} Let Assumption 1 hold, then
                \begin{align*}
                \underset{(x,\eta)\in \mathbb{R}^{n}\times\mathbb{Z}^{m-q}}{\text{minimize}} 
                & \enskip a^{T}x+d^{T}U_{2}\eta\\
                \text{subject to} 
                & \enskip Hx+BU_{2}\eta\leq  h -BU_{1}K^{-1}\theta.
              %  & \enskip y^{\ell}-U_{1}K^{-1}\theta \leq U_{2}\eta \leq y^{u}-U_{1}K^{-1}\theta.  
                \end{align*}
    \end{lem}
    \begin{IEEEproof}
        According to Proposition \ref{prop:propHermite}, the identity
        \begin{align*}
            y=U_{1}K^{-1}\theta+U_{2}\eta,
        \end{align*}
        holds. Therefore we can equivalently formulate Problem \ref{prob:Original-MILP} to 
        \begin{align*}
            \underset{(x,\eta)\in \mathbb{R}^{n}\times\mathbb{Z}^{m-q}}{\text{minimize}} 
            & \enskip a^{T}x+d^{T}U_{2}\eta\\
            \text{subject to} 
            & \enskip Hx+BU_{2}\eta\leq  h -BU_{1}K^{-1}\theta. \\
          %  & \enskip y^{\ell}-U_{1}K^{-1}\theta \leq U_{2}\eta \leq y^{u}-U_{1}K^{-1}\theta.  
            \end{align*}
        by substitution.
    \end{IEEEproof}
    Taking the reparameterized form from Lemma \ref{lem:reparam} we arrive at a continous linear programming problem that is guranteed to result in a feasible mixed integer solution.
    \begin{problem}
    \emph{(Feasible Reformulated LP)\label{prob:Feasible_LP}}
    \end{problem}
    \begin{align*}
        \underset{(x,\eta)\in \mathbb{R}^{n}\times\mathbb{R}^{m-q}}{\text{minimize}} 
        & \enskip a^{T}x+d^{T}U_{2}\eta\\
        \text{subject to} 
        & \enskip Hx+ BU_{2}\eta\leq \lfloor h -BU_{1}K^{-1}\theta\rfloor + \xi -\frac{1}{2}\|\beta 
         \|_{1}. \\
        % & \enskip y^{\ell}-U_{1}K^{-1}\theta -\delta \leq U_{2}\eta \leq y^{u}-U_{1}K^{-1}\theta+\delta.
        \end{align*}
    Round the optimal solution of $\eta$ and use the mapping 
    \begin{equation}\label{eq:yChangeOfVariables}
        y=U_{1}K^{-1}\theta+U_{2}\eta
    \end{equation}
    to obtain a feasible solution.
    \begin{problem}
        \emph{(Feasible R-LP Matrix Form)\label{prob:matrix_Feasible_LP}}
        \end{problem}
        \begin{align*}
            \underset{z}{\text{minimize}} 
            & \enskip c^{T}z\\
            \text{subject to} 
            & \enskip Az\leq b + \nu,
            \end{align*}
    
    \emph{where $z:=[x \enskip \eta]^{T}\in \mathbb{R}^{n\times(m-q)}$, $c:=[a\enskip (d^{T}U_{2})^{T}]\in \mathbb{R}^{n\times(m-q)}$, 
    $A := [H\enskip B]\in\mathbb{R}^{p\times (n+m)}$, $b := \lfloor h -BU_{1}K^{-1}\theta\rfloor\in\mathbb{R}^{p}$, $\nu := \xi -\frac{1}{2}\|\beta
    \|_{1}\in\mathbb{R}^{p}$, and the remapped solution is $\tilde{z} := [x \enskip U_{1}K^{-1}\theta+U_{2}\eta]^{T}\in \mathbb{R}^{n\times m}$.}
     \begin{prop}
        An MILP problem is granular if and only if there is a feasible point from the following feasibility problem
        \begin{align*}
            \underset{z}{\text{minimize}} 
            & \enskip 0\\
            \text{subject to} 
            & \enskip Az\leq b + \nu,
            \end{align*}
    where $\xi=0.9999$.

    \noindent \textbf{Assumption 2 (Nonempty and Compact) }\emph{The set
$Z$ is nonempty and compact.}

\noindent This assumption ensures the existence of a solution and
allows for distributed projected update laws which will ensure satisfaction
of the agents' set constraints.

\noindent \textbf{Assumption 3 (Slater's Condition)} \emph{Slater's
condition holds for $g,$} i.e., there exists $\bar{z}\in Z$ such
that $g(\bar{z})<0.$

\noindent This assumption will simplify our convergence analysis by
allowing us to formulate a saddle point problem over a compact domain. 

We solve Problem \ref{prob:matrix_Feasible_LP} using a primal-dual approach.
Specifically, we will use a decentralized form of the classic Uzawa
iteration, also called gradient descent-ascent, to find a saddle point
of the Lagrangian associated with Problem \ref{prob:matrix_Feasible_LP}.
This Lagrangian is $L(z,\lambda)=c^{T}z+\lambda^{T}(Az-b-\nu)$,
which is affine in both $z$ and $\lambda.$ Thus it is convex in
$z$ and concave in $\lambda.$ To ensure convergence of a decentralized
asynchronous implementation of the Uzawa iteration, we will regularize
$L$ to make it strongly convex in $z$ and strongly concave in $\lambda$.
These properties have both been shown to improve convergence of decentralized
algorithms \cite{koshal2011multiuser}. We apply a Tikhonov regularization
in the primal and dual spaces to find


\begin{align}
 & L_{\kappa}(z,\lambda)=c^{T}z+\frac{\alpha}{2}\vert\vert z\vert\vert^{2}+\lambda^{T}(Az-b-\nu)-\frac{\delta}{2}\vert\vert\lambda\vert\vert^{2},\label{eq:RegularizedLagran}
\end{align}
where $\lambda\in\mathbb{R}_{+}^{p}$ is the dual variable, $\alpha>0$
is the primal regularization term, $\delta>0$ is the dual regularization
term, and we use $\kappa=(\alpha,\delta$) to simplify notation. 

Strong duality holds for Problem \ref{prob:Relaxed-MILP} \cite[Section 5.2.3]{boyd2004convex},
which means it can be solved by computing the saddle point of the
unregularized Lagrangian $L$. Instead of doing so exactly, we will
compute a saddle point of the regularized Lagrangian $L_{\kappa}$
with $\alpha>0$ and $\delta>0$ set to small values. 

As we show in Section IV, this regularization
induces only minor error in the solutions we obtain. Another
advantage of regularizing is that we do not need to assume uniqueness
of the solution to Problem \ref{prob:Relaxed-MILP} since we have
strong convexity from regularization and thus $L_{\kappa}$ has a
unique saddle point. This is unlike existing large-scale MILP methods
that rely on assuming that there is a unique solution to solve Problem~\ref{prob:Relaxed-MILP}
\cite{camisa2021distributed,falsone2017dual,vujanic2016decomposition}.

Formally, we will solve Problem\ref{prob:Relaxed-MILP}
by finding a saddle point of $L_{\kappa}$, namely

\[
(\hat{z}_{\kappa},\hat{\lambda}_{\kappa})=\underset{z\in Z}{\text{arg min}}\underset{\lambda\in\mathbb{R}_{+}^{p}}{\enskip\text{arg max}}\enskip c^{T}z+\frac{\alpha}{2}\vert\vert z\vert\vert^{2}+\lambda^{T}(Az-b-\nu)-\frac{\delta}{2}\vert\vert\lambda\vert\vert^{2}.
\]
We next define a radius
$r$ to satisfy $Z\subseteq B_{o}(r)$. This value of $r$ is a bound
on the maximum norm of $z\in Z,$ and it can be found via
\begin{align}
r\triangleq\underset{z\in Z}{\max}\enskip & \vert\vert z\vert\vert.\label{eq:feasProblem-1}
\end{align}
\begin{lem}
\label{lem:saddlePoint}Let Assumptions 1 and 2 hold. Then

\[
\hat{\lambda}_{\kappa}\in M\triangleq\left\{ \lambda\in\mathbb{R}_{+}^{p}:\vert\vert\lambda\vert\vert_{1}\leq\frac{c^{T}\bar{z}+\frac{\alpha}{2}\vert\vert\bar{z}\vert\vert^{2}-\vert\vert c\vert\vert\cdot r}{\underset{1\leq j\leq m}{\min}-A_{row,j}\bar{z}-b_{j}-\nu_{j}}\right\} ,
\]
where $\bar{z}$ is a Slater point of $g$, \textup{$c^{T}\bar{z}$}
is the cost at the Slater point, $\alpha$ is the primal regularization
term, $r$ is the radius found from 
(\ref{eq:feasProblem-1}), $A_{row,j}$ denotes row $j$ of $A$,
and $-A_{j}\bar{z}-b_{j}-\nu_{j}$ is the $jth$ entry of $g(\bar{z})$.
\end{lem}
\begin{IEEEproof}
As discussed in \cite[Section II.C]{hale2015cloud} for any Slater
point $\bar{z}$ of $g$ we have

\begin{equation}
\hat{\lambda}_{\kappa}\in M\triangleq\left\{ \lambda\in\mathbb{R}_{+}^{y}:\vert\vert\lambda\vert\vert_{1}\leq\frac{f(\bar{z})+\frac{\alpha}{2}\vert\vert\bar{z}\vert\vert^{2}-\underset{z\in Z}{\min}f(z)}{\underset{1\leq j\leq m}{\min}-g_{j}(\bar{z})}\right\} .\label{eq:Lem4_part1}
\end{equation}
We expand $g(\bar{z})=A\bar{z}+-b-\nu$, which implies $g_{j}(\bar{z})=A_{j}\bar{z}-b_{j}-\nu_{j}.$
Then 
\begin{equation}
\underset{1\leq j\leq m}{\min}-g_{j}(\bar{z})=\underset{1\leq j\leq m}{\min}-A_{row,j}\bar{z}-b_{j}-\nu_{j}.\label{eq:Lem4_part2}
\end{equation}
Next, we find a lower bound for $\underset{z\in Z}{\min}f(z)$. It
follows that

\begin{equation}
\underset{z\in Z}{\min}\quad c^{T}z\geq\underset{z\in B_{o}(r)}{\min}c^{T}z=c^{T}\cdot\begin{pmatrix}-\frac{c}{\vert\vert c\vert\vert}\end{pmatrix}\cdot r=-\vert\vert c\vert\vert\cdot r.\label{eq:Lem4_part3}
\end{equation}
%where $r$ is from the feasibility problem in Eq. (\ref{eq:feasProblem-1}).
Substituting (\ref{eq:Lem4_part2}) and (\ref{eq:Lem4_part3})
into (\ref{eq:Lem4_part1}) gives the desired bound.
\end{IEEEproof}
We now bound the suboptimality in the primal component of the saddle
point of $L_{\kappa}$ that is due to the regularization of $L.$
Below, we will use this lemma to bound the suboptimality of the primal
component of the saddle point of $L_{\kappa}$, namely $\hat{z}_{\kappa}$,
relative to the optimal solution to Problem \ref{prob:Original-MILP}.
\begin{lem}
\label{lem:regError} Let Assumptions 1 and 2 hold.
Then

\[
    \vert c^{T}\hat{z}_{\kappa}-c^{T}z^{*}\vert\leq\vert\vert c\vert\vert\cdot\left(\frac{c^{T}\bar{z}+\frac{\alpha}{2}\vert\vert\bar{z}\vert\vert^{2}-\vert\vert c\vert\vert\cdot r}{\underset{1\leq j\leq m}{\min}-A_{row,j}\bar{z}-b_{j}-\nu_{j}}\right)\cdot\sqrt{\frac{\delta}{2\alpha}}+\frac{\alpha}{2}\cdot r,
\]
where $\hat{z}_{\kappa}$ is the primal component of the saddle point
of the regularized Lagrangian, $z^{*}$ is the primal component of
the saddle point of the unregularized Lagrangian~$L$,
$\bar{z}$ is a Slater point for $g$, $\alpha$ is the primal regularization
term, $\delta$ is the dual regularization term, $r$ is found from
 (\ref{eq:feasProblem-1}), and \textup{$-A_{j}\bar{z}-b_{j}-\nu_{j}$
is the explicit form of $-g_{j}(\bar{z})$.}
\end{lem}
\begin{IEEEproof}
From the general form presented in \cite[Lemma 3.3]{koshal2011multiuser},
we find an upper bound between the costs at $\hat{z}_{\kappa}$ and
$z^{*}$ via
\begin{equation}
\vert f(\hat{z}_{\kappa})-f(z^{*})\vert\leq\underset{z\in Z}{\max}\vert\vert\nabla f(z)\vert\vert\cdot\underset{\lambda\in M}{\max}\vert\vert\lambda\vert\vert\cdot\sqrt{\frac{\delta}{2\alpha}}+\frac{\alpha}{2}\cdot\underset{z\in Z}{\max}\vert\vert z\vert\vert.\label{eq:optBoundFull}
\end{equation}
From Problem \ref{prob:matrix_Feasible_LP}, we find
\[
\underset{z\in Z}{\max}\vert\vert\nabla f(z)\vert\vert=\vert\vert c\vert\vert,
\]
since $\nabla f \equiv c.$ Then we find an upper bound for $\underset{z\in Z}{\max}\vert\vert z\vert\vert$
as

\begin{equation}
\underset{z\in Z}{\max}\vert\vert z\vert\vert\leq\underset{z\in B_{o}(r)}{\max}\vert\vert z\vert\vert=r,\label{eq:maxR}
\end{equation}
which can be found explicitly from 
(\ref{eq:feasProblem-1}). Since $\ensuremath{\lambda}$ is a vector,
we always have $\underset{\lambda\in M}{\max}\vert\vert\lambda\vert\vert_{2}\leq\underset{\lambda\in M}{\max}\vert\vert\lambda\vert\vert_{1}.$
From Lemma 1, we can therefore upper bound $\vert\vert\lambda\vert\vert_{2}$
as
\begin{align}
 \underset{\lambda\in M}{\max}\vert\vert\lambda\vert\vert_{2} &\leq\underset{\lambda\in M}{\max}\left(\frac{c^{T}\bar{z}+\frac{\alpha}{2}\vert\vert\bar{z}\vert\vert^{2}-\vert\vert c\vert\vert\cdot r}{\underset{1\leq j\leq m}{\min}-A_{row,j}\bar{z}-b_{j}-\nu_{j}}\right) \\ &=\frac{c^{T}\bar{z}+\frac{\alpha}{2}\vert\vert\bar{z}\vert\vert^{2}-\vert\vert c\vert\vert\cdot r}{\underset{1\leq j\leq m}{\min}-A_{row,j}\bar{z}-b_{j}-\nu_{j}}.\label{eq:boundmaxLamb-1}
\end{align}
Then, using (\ref{eq:maxR}) and (\ref{eq:boundmaxLamb-1}) in (\ref{eq:optBoundFull}) we find
\begin{equation}
\vert c^{T}\hat{z}_{\kappa}-c^{T}z^{*}\vert\leq\vert\vert c\vert\vert\cdot\left(\frac{c^{T}\bar{z}+\frac{\alpha}{2}\vert\vert\bar{z}\vert\vert^{2}-\vert\vert c\vert\vert\cdot r}{\underset{1\leq j\leq m}{\min}-A_{row,j}\bar{z}-b_{j}-\nu_{j}}\right)\cdot\sqrt{\frac{\delta}{2\alpha}}+\frac{\alpha}{2}\cdot r.
\end{equation}
% Rearranging terms we have an upper bound on $c^{T}\hat{z}_{\kappa}$
% via 

% \[
% c^{T}\hat{z}_{\kappa}\leq c^{T}z^{*}+\vert\vert c\vert\vert\cdot\left(\frac{c^{T}\bar{z}+\frac{\alpha}{2}\vert\vert\bar{z}\vert\vert^{2}-\vert\vert c\vert\vert\cdot r}{\underset{1\leq j\leq m}{\min}-A_{row,j}\bar{z}-b_{j}-\nu_{j}}\right)\cdot\sqrt{\frac{\delta}{2\alpha}}+\frac{\alpha}{2}\cdot r.
% \]
Now that we have Lemma \ref{lem:saddlePoint}, and Lemma \ref{lem:regError}
, we construct the
suboptimality bound on the difference in optimal costs between Problem
\ref{prob:Original-MILP} and the primal component
of the regularized Lagrangian,~$\hat{z}_{\kappa}$.
\end{IEEEproof}
We can derive and upper bound on the optimality error between the rounded reparameterized optimal solution and the original mixed integer solution.
\begin{lem}
    \label{lem:Round}Let $z_{\text{\text{rounded}}}^{*}$ be
    the rounded optimal solution to the LP, $z^{*}$ be the non-rounded
    optimal solution to the LP, and c be the cost vector, then
    \end{lem}
    \[
    \vert c^{T}z_{\text{rounded}}^{*}-c^{T}z^{*}\vert\leq\frac{\vert\vert c\vert\vert_{2}}{2}.
    \]
    
    \begin{IEEEproof}
    The rounding upper bound is derived from a single line in the proof for \cite{stein2016error}[Lemma 3.6]. The proof follows 
    
    \[
    \vert c^{T}z_{\text{rounded}}^{*}-c^{T}z^{*}\vert\leq\vert\vert c\vert\vert_{2}\vert\vert z^{*}-z_{\text{rounded}}^{*}\vert\vert_{2}\leq\frac{\vert\vert c\vert\vert_{2}}{2}.
    \]
    \end{IEEEproof}
    \begin{lem}
    \label{lem:HoffmanError}Let $X=\mathbb{R}^{n},$ and let $\sigma$
    denote a Hoffman constant of a system of inequalities for $Av\leq b $ and let $\rho=1$.
    Then for all $\varsigma\in(0,\bar{\varsigma}]$ the rounding's optimality error satisfies
    
    \[
        \vert c^{T}v^{*}-c^{T}z_{\text{rounded}}^{*}\vert\leq(\vert\vert c\vert\vert_{2}(\sigma\vert\vert A_{\text{integer}}\vert\vert_{\infty}+1)+\vert\vert c_{\text{integer}}\vert\vert_{2})\frac{1}{2}+c_{\text{integer}}^{T}U_{1}K^{-1}h,
    \]
    where $X$ is the continous decision variable set constraint, $v:=[x \enskip y]^{T}$, $c_{\text{integer}}$ is the integer part of the objective function vector, and $A_{\text{integer}}$ is the integer part of the constraint matrix.
    \end{lem}
    \begin{IEEEproof}
    From \cite{stein2016error}[Theorem 4.4] the rounding optimality error satisfies,
    
    \[
    \vert c^{T}[x^{*}\enskip \eta_{\text{integer}}^{*}]^{T}-c^{T}z_{\text{rounded}}^{*}\vert\leq(\vert\vert(c,d)\vert\vert^{*}(\sigma\vert\vert A_{\text{integer}}\vert\vert_{\infty}+\rho)+\vert\vert d\vert\vert^{*}\rho)\frac{\varsigma}{2}.
    \]
    
    From Problem 2, this simplifies to 
    
    \begin{equation}\label{eq:hoffLemmaPart1}
    \vert c^{T}[x^{*}\enskip \eta_{\text{integer}}^{*}]^{T}-c^{T}z_{\text{rounded}}^{*}\vert\leq(\vert\vert c\vert\vert_{2}(\sigma\vert\vert A_{\text{integer}}\vert\vert_{\infty}+1)+\vert\vert c_{\text{integer}}\vert\vert_{2}\cdot 1)\frac{1}{2}.
    \end{equation}
    Subsequently, the optimal solution of the original MILP and the MILP with no equality constraints Eq. \ref{eq:yChangeOfVariables}
    \begin{equation}\label{eq:hoffLemmaPart2}
    \vert c^{T}v^{*}\enskip -c^{T}z_{\text{rounded}}^{*}\vert\leq c_{\text{integer}}^{T}U_{1}K^{-1}h.
    \end{equation}
    Summing the upper bound from Eq. \ref{eq:hoffLemmaPart1} and Eq. \ref{eq:hoffLemmaPart2} completes the proof.
    \end{IEEEproof}

    \begin{thm}(Suboptimality Error Bound)
        Let $z_{\text{rounded}}^{*}$ be the rounded optimal solution to the
        continuous LP, $z_{\kappa}^{*}$ be the optimal solution to the regularized continuous LP, $v^{*}$ be the optimal MILP
        solution, and $z^{*}$ be the optimal solution to the continous LP. Let $\sigma$ be the Hoffman constant.
        Then,
        \[
            \vert c^{T}v^{*}-c^{T}z_{\kappa}^{*}\vert \leq + (\vert\vert c\vert\vert_{2}(\sigma\vert\vert A_{\text{integer}}\vert\vert_{\infty}+1)+\vert\vert c_{\text{integer}}\vert\vert_{2})\frac{1}{2}+c_{\text{integer}}^{T}U_{1}K^{-1}h + \vert\vert c\vert\vert\cdot\Gamma\cdot\sqrt{\frac{\delta}{2\alpha}}+\frac{\alpha}{2}\cdot r,
        \]
        where $\Gamma = \left(\frac{c^{T}\bar{z}+\frac{\alpha}{2}\vert\vert\bar{z}\vert\vert^{2}-\vert\vert c\vert\vert\cdot r}{\underset{1\leq j\leq m}{\min}-A_{row,j}\bar{z}-b_{j}-\nu_{j}}\right).$
       
        \end{thm}
        \begin{IEEEproof}
        Take $\vert c^{T}v^{*}-c^{T}z_{\kappa}^{*}\vert,$
        and apply the triangle inequality
        
        \[
        \vert(c^{T}v^{*}-c^{T}z_{\text{rounded}}^{*})+(c^{T}z_{\text{rounded}}^{*}-c^{T}z^{*})+(c^{T}z^{*}-c^{T}z_{\kappa}^{*})\vert\leq\vert c^{T}v^{*}-c^{T}z_{\text{rounded}}^{*}\vert+\vert c^{T}z_{\text{rounded}}^{*}-c^{T}z^{*}\vert+\vert c^{T}z^{*}-c^{T}z_{\kappa}^{*}\vert
        \]
        
        simplifies to
        
        \[
        \vert c^{T}v^{*}-c^{T}z_{\kappa}^{*}\vert\leq\vert c^{T}v^{*}-c^{T}z_{\text{rounded}}^{*}\vert+\vert c^{T}z_{\text{rounded}}^{*}-c^{T}z^{*}\vert+\vert c^{T}z^{*}-c^{T}z_{\kappa}^{*}\vert.
        \]
        
        From Lemma (\ref{lem:Round}), 
        
        \begin{equation}
        \vert c^{T}z_{\text{rounded}}^{*}-c^{T}z^{*}\vert\leq\frac{\vert\vert c\vert\vert_{2}}{2}.\label{eq:ubZroundToZ*}
        \end{equation}
        
        From Lemma (\ref{lem:HoffmanError}),
        
        \begin{equation}
            \vert c^{T}v^{*}-c^{T}z_{\text{rounded}}^{*}\vert\leq(\vert\vert c\vert\vert_{2}(\sigma\vert\vert A_{\text{integer}}\vert\vert_{\infty}+1)+\vert\vert c_{\text{integer}}\vert\vert_{2})\frac{1}{2}+c_{\text{integer}}^{T}U_{1}K^{-1}h.\label{eq:ubZRounded}
        \end{equation}
        
        From Lemma (\ref{lem:regError}),
        
        \begin{equation}
            \vert c^{T}\hat{z}_{\kappa}-c^{T}z^{*}\vert\leq\vert\vert c\vert\vert\cdot\left(\frac{c^{T}\bar{z}+\frac{\alpha}{2}\vert\vert\bar{z}\vert\vert^{2}-\vert\vert c\vert\vert\cdot r}{\underset{1\leq j\leq m}{\min}-A_{row,j}\bar{z}-b_{j}-\nu_{j}}\right)\cdot\sqrt{\frac{\delta}{2\alpha}}+\frac{\alpha}{2}\cdot r.\label{eq:ubZreg}
        \end{equation}
        
        Summing the upper bounds for the three difference terms Eq. (\ref{eq:ubZroundToZ*}), (\ref{eq:ubZRounded}),
        and (\ref{eq:ubZreg}) completes the proof.
        \end{IEEEproof}
        \begin{thm}(Feasibility Error Bound)
            The solution is feasible at optimality so error bound should just be due to regularization and or use Stein EB for fun.
        \end{thm}
        \begin{IEEEproof}
            WIP
        \end{IEEEproof}
     \end{prop}
